Personalized Attacks of Social Engineering in Multi-turn Conversations: LLM Agents for Simulation and Detection

The rapid advancement of conversational agents, particularly chatbots powered by Large Language Models (LLMs), poses a significant risk of social engineering (SE) attacks on social media platforms. SE detection in multi-turn, chat-based interactions is considerably more complex than single-instance detection due to the dynamic nature of these conversations. A critical factor in mitigating this threat is understanding the SE attack mechanisms through which SE attacks operate, specifically how attackers exploit vulnerabilities and how victims' personality traits contribute to their susceptibility. In this work, we propose an LLM-agentic framework, SE-VSim, to simulate SE attack mechanisms by generating multi-turn conversations. We model victim agents with varying personality traits to assess how psychological profiles influence susceptibility to manipulation. Using a dataset of over 1000 simulated conversations, we examine attack scenarios in which adversaries, posing as recruiters, funding agencies, and journalists, attempt to extract sensitive information. Based on this analysis, we present a proof of concept, SE-OmniGuard, to offer personalized protection to users by leveraging prior knowledge of the victims personality, evaluating attack strategies, and monitoring information exchanges in conversations to identify potential SE attempts.

==> content/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\paragraph{Human-Initiated Social Engineering Defense}
SE attacks are frequently carried out through communication mediums like SMS, phone calls, and online chat platforms, including social media channels \cite{tsinganos2018towards, zheng2019session}. Researchers have extensively mapped the various phases of SE attacks \cite{zheng2019session, wang2021social, karadsheh2022impact}, which have informed the development of several defense mechanisms. For instance, \citet{lansley2020seader++} developed SEADER++, an SE detection system in online chat environments, which leverages synthetic datasets and an MLP classifier to identify malicious dialogues. Similarly, \citet{yoo2022icsa} proposed ICSA, a chatbot security assistant that employs TextCNN-based classifiers to detect different stages of phishing attacks on social networking services (SNS), offering targeted defensive interventions. More recent advancements include fine-tuned models for SE dialogue tracking. For example, \citet{tsinganos2022applying} applied BERT on the CSE-Persistence corpus, while \citet{tsinganos2023leveraging} introduced SG-CSE BERT for zero-shot SE attack detection in dialogue-state tracking. CSE-ARS \cite{tsinganos2024cse}, a late-fusion model, combined outputs from five deep learning models to identify diverse SE attack vectors, enhancing detection accuracy across multiple contexts.

\paragraph{Personality Traits and Susceptibility in SE Attacks}
Individual differences in personality traits pose challenges for organizations in designing effective strategies to prevent phishing attacks \cite{anawar2019analysis}. Research has consistently demonstrated that personality traits can significantly affect a person’s susceptibility to manipulation \cite{rahman2022discovering}. Studies using models like the Big Five personality traits \cite{cusack2019impact} have shown that individuals with certain characteristics, such as high agreeableness or low conscientiousness, are more likely to fall victim to phishing and other forms of deception \cite{7497779, anawar2019analysis}. As a result, integrating personality recognition into defense systems has proven effective in improving the detection of manipulation and deception \cite{an2018deep}. Despite this, most SE defense systems still treat all users with a one-size-fits-all approach, neglecting the impact of individual personality differences. To address this limitation, our work introduces personality-aware simulations to model victim agents with varying psychological traits. By leveraging the persona simulation capabilities of LLMs \cite{hu2024quantifying, schuller2024generating, sun2024building}, we aim to gain a deeper understanding of how these traits affect susceptibility to manipulation.

\paragraph{LLM Agents and Cyber-Attacks} 
While traditional SE defenses primarily focus on human-initiated attacks, the rapid growth of LLMs introduces novel threats. LLMs, capable of mimicking human conversational patterns, trust cues \cite{mireshghallahtrust, hua2024trustagent}, and eliciting emotions \cite{miyakawa-etal-2024-llms, gong-etal-2023-eliciting}, creating new opportunities for sophisticated digital deception \cite{wu-etal-2024-deciphering, schmitt2023digital, glenski2020user, ai2021exploring, ai2022combating, kumarage2024survey, beigi2024lrq} and SE attacks \cite{schmitt2023digital}. Although there are efforts to simulate cyberattacks using LLMs \cite{xu2024autoattacker, happe2023getting, naito2023llm, fang2024llm, kumarage2023reliable}, the specific domain of LLM-driven SE attacks remains underexplored. \citet{asfour2023harnessing} began modeling human responses to SE attacks via LLMs, but comprehensive frameworks addressing multi-turn conversations and psychological dynamics are still in their infancy. \citet{ai2024defending} represents a key step forward by investigating how LLMs can serve as both a facilitator and a defense mechanism against SE attacks. However, this work overlooks the impact of victim personality traits on susceptibility. Our work introduces a novel contribution by integrating personality-aware defense strategies, paving the way for personalized protection systems that dynamically assess and respond to potential LLM-powered SE threats.

==> content/results.tex <==

\begin{table}[h!]
    \centering
    \resizebox{.5\textwidth}{!}{
    \begin{tabular}{|l|l|cccc|cccc|}
    \hline
    \multirow{2}{*}{LLM} & \multirow{2}{*}{Approach} & \multicolumn{4}{c|}{Accuracy} & \multicolumn{4}{c|}{F1} \\
     &  & AF & JO & RE & Overall & AF & JO & RE & Overall \\ 
     \hline
    \multirow{5}{*}{Llama 3} 
     & Zero-Shot     & 0.487 & 0.470 & 0.460 & 0.472 & 0.487 & 0.478 & 0.449 & 0.472 \\ 
     & AF Few-Shot   & 0.717 & 0.677 & 0.700 & 0.698 & 0.814 & 0.790 & 0.805 & 0.803 \\
     & JO Few-Shot   & 0.663 & 0.690 & 0.650 & 0.668 & 0.763 & 0.792 & 0.767 & 0.774 \\ 
     & RE Few-Shot   & 0.720 & 0.783 & 0.775 & 0.790 & 0.813 & 0.783 & 0.775 & 0.790 \\ 
     & ConvoSentinel & 0.59 & 0.43 & 0.55 & 0.53 & 0.59 & 0.40 & 0.55 & 0.52 \\ 
     \hline
    \multirow{5}{*}{GPT-4o} 
     & Zero-Shot     & 0.500 & 0.363 & 0.463 & 0.442 & 0.400 & 0.086 & 0.326 & 0.281 \\ 
     & AF Few-Shot   & 0.597 & 0.453 & 0.617 & 0.556 & 0.572 & 0.305 & 0.596 & 0.502 \\
     & JO Few-Shot   & 0.630 & 0.473 & 0.577 & 0.560 & 0.621 & 0.347 & 0.538 & 0.511 \\
     & RE Few-Shot   & 0.587 & 0.440 & 0.623 & 0.550 & 0.557 & 0.276 & 0.609 & 0.494 \\ 
     & ConvoSentinel & 0.63 & 0.50 & 0.64 & 0.59 & 0.62 & 0.45 & 0.63 & 0.57 \\ 
     \hline
     % \multirow{5}{*}{Mistral} 
     % & Zero-Shot     &  &  &  &  &  &  &  &  \\ 
     % & AF Few-Shot   &  &  &  &  &  &  &  &  \\ 
     % & JO Few-Shot   &  &  &  &  &  &  &  &  \\ 
     % & RE Few-Shot   &  &  &  &  &  &  &  &  \\ 
     % & ConvoSentinel &  &  &  &  &  &  &  &  \\ 
     % \hline
     \multirow{1}{*}{{GPT-4o}} & {\Model} & 0.82 & 0.81  & 0.83 & 0.82 & 0.78 & 0.80  & 0.82 & 0.80 \\ 
    \hline
    \end{tabular}
    }
    \caption{Baseline ablation and generalization: the baselines were trained using only the AF data, the JO data, and the RE data, respectively. Then each of those models was evaluated against the data class they were trained on, as well as the two unseen data classes.} \label{tab:baselines}
\end{table} 

% Old
% \begin{table}[h!]
%     \centering
%     \resizebox{.5\textwidth}{!}{
%     \begin{tabular}{|l|l|cccc|cccc|}
%     \hline
%     \multirow{2}{*}{LLM} & \multirow{2}{*}{Approach} & \multicolumn{4}{c|}{Accuracy} & \multicolumn{4}{c|}{F1} \\
%      &  & AF & JO & RE & Overall & AF & JO & RE & Overall \\ 
%      \hline
%     \multirow{5}{*}{Llama3-8B} 
%      & Zero-Shot     & 0.487 & 0.470 & 0.460 & 0.487 & 0.479 & 0.472 & 0.449 & 0.472 \\ 
%      & AF Few-Shot   & 0.390 & 0.407 & 0.367 & 0.388 & 0.271 & 0.305 & 0.240 & 0.272 \\
%      & JO Few-Shot   & 0.443 & 0.363 & 0.383 & 0.397 & 0.369 & 0.220 & 0.239 & 0.279\\
%      & RE Few-Shot   & 0.380 & 0.400 & 0.393 & 0.391 & 0.250 & 0.268 & 0.272 & 0.263 \\
%      & ConvoSentinel &  &  &  & 0.53 &  &  &  & 0.52 \\ 
%      \hline
%     \multirow{5}{*}{gpt-4o-mini} 
%      & Zero-Shot     & 0.500 & 0.363 & 0.463 & 0.442 & 0.400 & 0.086 & 0.326 & 0.281 \\ 
%      & AF Few-Shot   & 0.597 & 0.453 & 0.617 & 0.556 & 0.572 & 0.305 & 0.596 & 0.502 \\
%      & JO Few-Shot   & 0.630 & 0.473 & 0.577 & 0.560 & 0.621 & 0.347 & 0.538 & 0.511 \\
%      & RE Few-Shot   & 0.587 & 0.440 & 0.623 & 0.550 & 0.557 & 0.276 & 0.609 & 0.494 \\ 
%      & ConvoSentinel &  &  &  &  &  &  &  &  \\ 
%      \hline
%      \multirow{5}{*}{Mistral} 
%      & Zero-Shot      \\ 
%      & AF Few-Shot    \\
%      & JO Few-Shot    \\
%      & RE Few-Shot    \\ 
%      & ConvoSentinel &  &  &  &  &  &  &  &  \\ 
%      \hline

%     \end{tabular}
%     }
%     \caption{Baselines ablation and generalization: the baselines were trained using only the AF data, the JO data, and the RE data, respectively. Then each of those models was evaluated against the data class they were trained on, as well as the two unseen data classes.} \label{tab:baselines}
% \end{table} 

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

